A study of gamma-ray emission from OJ 287 using Fermi-LAT from 2015-2023

We search for gamma-ray emission from OJ287 in the energy range from 0.1-300 GeV during 2015-2023, in coincidence with an extensive observing campaign to monitor the optical flux variability and polarization, as discussed in arXiv:2311.02372. We present results for eight segments in the aforementioned period, with each segment corresponding to an observing season. We report non-zero gamma-ray flux (with $>10\sigma$ significance) for all the eight segments. The photon and energy flux observed during this period is $\sim 5.2 \times 10^{-8} \rm{ph~cm^{-2}~s^{-1}}$ and $2.75 \times 10^{-5} \rm{MeV~cm^{-2}~s^{-1}}$, respectively, while the SED can be fitted with a power law with a slope of $2.12 \pm 0.02$. The observed luminosity is between $10^{45}-10^{46}$ ergs/sec. Similar to previous works we find a hard cutoff in the gamma-ray spectrum at around 20 GeV. We do not observe any correlations between the peaks in the gamma ray light curves and corresponding optical light cuves in $I$ and $R$ bands, as well as the X-ray light curves from SWIFT between 0.3-10 keV.

==> Img/Target_results.tex <==
\begin{tabular}{llllll}
\toprule
 & TS & Flux & EnergyFlux & N0 (log scale) & Alpha \\
\midrule
1 &  1586.61 &  1.079e-07 +/- 7.01e-09 &  4.649e-05 +/- 2.65e-06 &  -9.508785396808392 - 0.025346760221438558 + 0.02516957598513514 &  2.13689226864109 - 0.03923360332184256 + 0.03940377730250644 \\
2 &  891.89 &   4.07e-08 +/- 5.33e-10 &  3.524e-05 +/- 9.28e-07 &  -9.940297534308906 - 0.05007516622809405 + 0.04985845179792214 &  1.9195345587612285 - 0.05416570828877809 + 0.05419983299168307 \\
3 &  155.29 &  3.438e-08 +/- 9.51e-09 &  1.532e-05 +/- 2.62e-06 &  -9.890805803230249 - 0.16023017714912768 + 0.15863057717766438 &  2.185727275805117 - 0.1921261239735199 + 0.19208030215530636 \\
3 &  154.60 &  3.882e-08 +/- 6.69e-09 &  1.862e-05 +/- 3.34e-06 &  -10.059149633555567 - 0.11683503605392076 + 0.11751751806869315 &  1.9671892481291455 - 0.12374872434707251 + 0.12233342081737542 \\
4 &  263.04 &    4.8e-08 +/- 7.84e-09 &  2.015e-05 +/- 3.38e-06 &  -9.903531353933015 - 0.06134593699534818 + 0.060651902354061704 &  2.213552321146212 - 0.09654588041415524 + 0.09632666702855097 \\
5 &  379.65 &  4.524e-08 +/- 7.21e-09 &  2.602e-05 +/- 4.53e-06 &  -9.960613402204995 - 0.05101534454042245 + 0.04981683837348605 &  2.098406814654115 - 0.0651404095579089 + 0.0645865226615161 \\
6 &  308.48 &  3.715e-08 +/- 6.68e-09 &  2.055e-05 +/- 3.32e-06 &  -9.962487259040131 - 0.06249771178922359 + 0.06062813634584785 &  2.0361209256062183 - 0.08057099348653107 + 0.07903077702469119 \\
7 &  320.09 &  2.063e-08 +/- 2.45e-09 &  1.945e-05 +/- 2.72e-06 &  -10.19612152326851 - 0.12364809458249582 + 0.12674742292382213 &  1.8450902341522157 - 0.11438361664420094 + 0.11724425536242289 \\
a &  4774.88 &  5.176e-08 +/-  4.7e-10 &  2.745e-05 +/- 3.75e-07 &  -9.856321919506538 - 0.014931771945782657 + 0.014977790186604167 &  2.120902235877108 - 0.018754351727962693 + 0.019140905863530566 \\
t &  771.98 &  4.703e-08 +/- 5.22e-09 &  1.925e-05 +/- 1.52e-06 &  -9.893922194784935 - 0.03749332259319793 + 0.03727607544787048 &  2.0391916090190665 - 0.12905551938359539 + 0.13162372539940925 \\
\bottomrule
\end{tabular}

